Testing Individual Fairness in Graph Neural Networks

The biases in artificial intelligence (AI) models can lead to automated decision-making processes that discriminate against groups and/or individuals based on sensitive properties such as gender and race. While there are many studies on diagnosing and mitigating biases in various AI models, there is little research on individual fairness in Graph Neural Networks (GNNs). Unlike traditional models, which treat data features independently and overlook their inter-relationships, GNNs are designed to capture graph-based structure where nodes are interconnected. This relational approach enables GNNs to model complex dependencies, but it also means that biases can propagate through these connections, complicating the detection and mitigation of individual fairness violations. This PhD project aims to develop a testing framework to assess and ensure individual fairness in GNNs. It first systematically reviews the literature on individual fairness, categorizing existing approaches to define, measure, test, and mitigate model biases, creating a taxonomy of individual fairness. Next, the project will develop a framework for testing and ensuring fairness in GNNs by adapting and extending current fairness testing and mitigation techniques. The framework will be evaluated through industrial case studies, focusing on graph-based large language models.

==> Background.tex <==
\section{Background}

\subsection{Fairness in AI Models}


Fairness generally implies the absence of prejudice or favoritism towards any individual or group based on their inherent or acquired characteristics~\cite{mehrabi2022survey}. There are two main categories: group and individual fairness~\cite{dwork2011fairnessawareness}.

Group fairness ensures that instances from different groups receive similar treatment. While this guarantees fair outcomes at the group level, it does not necessarily prevent discriminatory treatment of individuals or subgroups within a protected category~\cite{dwork2011fairnessawareness}. To address this limitation, Dwork et al. introduced the concept of individual fairness, which requires that similar individuals receive similar predictions. To clarify this concept, let us consider an example:

The Adult dataset~\footnote{https://archive.ics.uci.edu/dataset/2/adult} contains census information of individuals used to determine if an individual can earn more than \$50K per year. The dataset includes 13 attributes. Two protected attributes are present in the dataset: Gender and Race. Now, we can apply the concepts of individual and group fairness to evaluate the fairness of predictions, such as predicting whether an individual earns more than \$50K per year. 

One common approach to group fairness is demographic parity, which aims for equal acceptance rates across different groups. 

For example, gender (male and female) can be considered a protected attribute. If the prediction model is designed to predict whether an individual earns more than \$50K per year, group fairness in this context would mean that the proportion of males and females predicted to earn more than \$50K should be roughly the same. If 40\% of males are predicted to earn more than \$50K, 40\% of females should also be predicted to earn more than \$50K to ensure demographic parity. If the model predicts a much higher percentage of males than females as high-earners, the model would violate group fairness (Figure~\ref{fig:groupfairness}).

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.50\textwidth]{Figures/GF.png} 
    \caption{Group Fairness}
    \label{fig:groupfairness}
\end{figure}


For individual fairness, consider two individuals:

Individual 1: A 35-year-old woman with a bachelor’s degree, working as a software engineer for 8 years, earning \$60K.\\
Individual 2: A 35-year-old man with a bachelor’s degree, working as a software engineer for 8 years, earning \$60K.

If the model predicts that Individual 1 will earn more than \$50 K but predicts that Individual 2 will earn less than \$50K, this violates individual fairness. Even though their features (age, education, years of experience, and job role) are nearly identical, the model gives different predictions, which is unfair to Individual 1 and Individual 2 under the individual fairness criterion (Figure~\ref{fig:individualfairness}).

\begin{figure}[!ht]
\centering
\includegraphics[width=0.50\textwidth]{Figures/IF.png}
\caption{Individual Fairness}
\label{fig:individualfairness}
\end{figure}

Both concepts are essential in evaluating fairness in machine learning systems, but they address different dimensions of fairness. Group fairness may overlook disparities within protected groups, while individual fairness ensures that those who are similarly situated are treated equitably, regardless of their group affiliation. Balancing both types of fairness is critical for creating more comprehensive and just ML models.

\subsection{Graph Neural Networks}

GNNs are a type of deep learning model designed to handle graph-structured data, which is common in many real-world applications, such as social networks, molecular chemistry, and recommendation systems~\cite{Jiawen2023recommneders}. Unlike traditional deep learning models that operate on grid-like data (such as images or text), GNNs work by capturing the relationships and dependencies between entities (nodes) represented as graphs. In a GNN, each node aggregates information from its neighboring nodes to update its feature representation. Mathematically, the feature representation of a node $v$ at the $k$-th layer, denoted $h_v^{(k)}$, is updated by aggregating the features of its neighbors $N(v)$ and applying a transformation to its own features. This can be expressed as:

\[
h_v^{(k+1)} = \text{Aggregation}\left( \{ h_u^{(k)} \mid u \in N(v) \} \right) + W^{(k)} h_v^{(k)}
\]

Where $N(v)$ is the set of neighboring nodes of $v$, and $W^{(k)}$ is the learnable weight matrix at the $k$-th layer. The aggregation function combines the features from the neighboring nodes, and the updated feature $h_v^{(k+1)}$ represents a blend of both the node’s own features and the information from its local network. This process enables GNNs to model interconnected data by combining node features and graph structure, efficiently processing data while preserving spatial and relational information~\cite{Dong2021REDRESS}.

Concerning fairness, GNNs introduce unique challenges compared to other deep learning models~\cite{Dong2023GM}. In traditional neural networks, fairness concerns typically arise from biased training data or algorithmic decisions based on biased features. However, GNNs have the added complexity of fairness issues embedded within the graph structure itself. For example, if specific nodes with sensitive attributes (like gender or race) are more likely to be connected to each other, GNNs can unintentionally learn biased representations due to the homophily effect, where similar nodes are connected. This can perpetuate and amplify biases, leading to unfair outcomes. Moreover, the diffusion of information across the graph can spread sensitive attribute correlations, further complicating fairness mitigation. Unlike standard deep learning methods, GNNs require novel approaches to ensure fairness, such as accounting for biased graph structures and carefully handling feature diffusion to avoid perpetuating discrimination~\cite{Dong2023GM}.


